Heuristic Search for Path Finding with Refuelling

This paper considers a generalization of the Path Finding (PF) problem with refuelling constraints referred to as the Gas Station Problem (GSP). Similar to PF, given a graph where vertices are gas stations with known fuel prices, and edge costs are the gas consumption between the two vertices, GSP seeks a minimum-cost path from the start to the goal vertex for a robot with a limited gas tank and a limited number of refuelling stops. While GSP is polynomial-time solvable, it remains a challenge to quickly compute an optimal solution in practice since it requires simultaneously determine the path, where to make the stops, and the amount to refuel at each stop. This paper develops a heuristic search algorithm called Refuel A$^*$ (RF-A$^*$) that iteratively constructs partial solution paths from the start to the goal guided by a heuristic while leveraging dominance rules for pruning during planning. RF-A$^*$ is guaranteed to find an optimal solution and often runs 2 to 8 times faster than the existing approaches in large city maps with several hundreds of gas stations.

==> Extra/Related_works.tex <==

\section{Related Work}
\label{ppwr:sec:Related}

\subsection{Resource-Constrained Shortest Path Problems (RCSPP):}
The Resource Constrained Shortest Path Problem (RCSPP) asks for the computation of a ''least cost'' path obeying a set of resource constraints between some start and destination locations. We are given a graph $G(V,E)$ where $V$ is the set of vertices, and $E$ is the set of edges, a source node $s$ and a target node $t$ and $k$ resource limits  $\lambda^{(1)}$ to $\lambda^{(k)}$. Each of the edges ($e$) have some cost $c_e$ and consume some ${r_e}^{i}$ of resource $i$, where $1\leq i \leq k$. The costs and resources usages are assumed to be non-negative and additive along the paths. Given some source node $s$ and destination node $t$, RCSPP aims to find a path ${\Pi_{st}}^{*}$ such that $c({\Pi_{st}^{*}}) \leq c({\Pi_{st}})$ for each path $\Pi_{st}$ in $G$ and the optimal path ${\Pi_{st}^{*}}$ must satisfy all feasibility criterion associated with each resource.Various methods have been proposed to tackle these problems, including dynamic programming \cite{irnichShortestPathProblems2005}, path ranking \cite{puglieseSurveyResourceConstrained2013, mehlhornResourceConstrainedShortest2000}, Lagrangian relaxation \cite{puglieseSurveyResourceConstrained2013}, Label-Setting and Label-Correcting Algorithms \cite{puglieseSurveyResourceConstrained2013}, and Reinforcement Learning \cite{ottoniReinforcementLearningTraveling2022}. RCSPP research holds significant importance in multi-agent systems, robotics, and transportation networks, and many studies have focused on developing efficient algorithms and techniques to address these challenges.

% The resource-constrained path problem is a broad set of problems that can be divided into four main groups [3]: (1) Shortest Path Problem With Time Windows, (2) Resource-constrained Shortest Path Problem, (3) Resource-constrained Elementary Shortest Path Problem, and (4) Shortest Path Problems with Forbidden Paths. 
\subsection{Multi-Objective Path Finding:}
The gas station problem, augmented with a constraint on the number of stops \cite{khullerFillNotFill2011}, introduces a multi-objective dimension, particularly due to the dual objectives of minimizing the costs and adhering to the limited number of stops allowed. However, our paper narrows its focus to a specific objective: minimizing the agent's energy refuelling costs. As a result, we address it as a \textit{single-objective path-finding problem}, emphasizing the optimization of refuelling expenses in the context of RCSPP. 

\subsection{Gas Station Problem:}
% \textcolor{red}{\textbf{DOUBT:} 
% \begin{enumerate}
%     \item should I expand on the work done here, for example, write more about the TSPWR, and papers which address the problem for a fixed route?
%     \item Should I also write about the 4 different problems mentioned in the S.Khuller paper?
% \end{enumerate}
% }

% The gas station problem, introduced in the paper [2], is a form of RCSPP where we need to consider the agent's fuel/energy levels and restrict the number of stops while minimizing the cost of refuelling throughout the chosen path. This problem has attracted significant attention in the field of optimization and algorithm design. S. Khuller's original work proposed a dynamic programming algorithm that efficiently solves the gas station problem in polynomial time. The algorithm identifies key states and transitions, representing different fuel levels at each gas station. However, due to its computational complexity, the dynamic programming approach may not be suitable for real-time applications or large-scale instances.

The gas station problem, introduced in the paper \cite{khullerFillNotFill2011}, is a form of Resource-Constrained Shortest Path Problem (RCSPP). It involves considering the agent's fuel/energy levels and limiting the number of stops while minimizing refuelling costs along the chosen path. This problem has garnered considerable attention in the field of optimization and algorithm design. S. Khuller's original work proposed a dynamic programming algorithm that efficiently solves the gas station problem in polynomial time with respect to the number of gas stations and fuel levels. The algorithm identifies key states and transitions, representing different fuel levels at each gas station.

However, it is important to clarify that while the dynamic programming algorithm is considered polynomial in the input size (number of gas stations and fuel levels), it may still exhibit high computational complexity for certain scenarios. Thus, in practical terms, it may not be suitable for real-time applications or large-scale instances where efficiency is critical. Alternative heuristic-based approaches, like the one proposed in our paper, are being explored to address the gas station problem more efficiently and effectively in such cases.s

Similar problems related to the gas station problem include the Electric Vehicle Touring Problem \cite{liaoElectricVehicleTouring2016}, the EV Recharging Problem, or the Vehicle Routing Problem \cite{liaoElectricVehicleTouring2016,swedaOptimalRechargingPolicies2017}. These problems involve a modified version of the Traveling Salesman Problem, incorporating recharging, fuel conservation, and fixed stop constraints. They are often tackled using various approaches, such as Dynamic Programming \cite{khullerFillNotFill2011}, Greedy Algorithms \cite{linFindingOptimalRefueling}, Reinforcement Learning (e.g., Q-learning and SARSA) \cite{ottoniReinforcementLearningTraveling2022}, Heuristic Techniques \cite{pourazarmOptimalRoutingEnergyAware2018}, and Online learning algorithms \cite{liOnlineRoutingAutonomous2022}.

Our paper addresses a more general version of the gas station problem, where the number of stops the agent can make is "unbounded." In other words, the agent does not need to concern itself with the number of stops but rather aims to minimize the cost of refuelling while travelling through the graph. To achieve this, we adopt a heuristic approach over the dynamic programming method, incorporating additional ideas of labels, pruning, and a frontier set to compute the optimal solution more efficiently, as detailed in Section V.




==> Extra/Sim_paper.tex <==
\section{Similar Work}

\subsection{Time Optimal routing of electric vehicles under consideration of Available Charging infrastructure and a Detailed Consumption Model} \cite{morlockTimeOptimalRouting2020}
This paper proposes a two-staged approach to compute time optimal routes for electric vehicles (EVs) by considering the available charging infrastructure in route planning and using a detailed powertrain model to forecast an EV's energy consumption accurately. The study aims to address EV drivers' range anxiety concerns and improve consumption forecast models' accuracy. The proposed methodology solves the resulting multiobjective shortest path problem using an adapted Moore-Bellman-Ford algorithm. The algorithm is adapted to handle the constraints of the EV routing problem, such as the limited battery capacity, present charging infrastructure, and intentional reduction of highway cruising speed to evade long charging times. The paper provides an algorithm for the adapted MBF algorithm. The consumption forecast is validated against measurement data, and the query times of the proposed methodology are assessed for generic routing problems. 

\subsection{The Electric Vehicle Touring} \cite{liaoElectricVehicleTouring2016}
The focus of this paper is on the fuel efficiency of EVs. The authors study EV routing problems that consider battery charging/swapping. The objective is to determine the shortest travel time route a vehicle with a given battery capacity can take to travel between a pair of vertices or visit a set of vertices with several stops, if necessary, at battery switch stations. The paper presents polynomial time algorithms for the EV shortest travel time path problem and the fixed tour EV touring problem, where the fixed tour problem requires visiting a set of vertices in a given order. Based on the results, the authors propose constant factor approximation algorithms for the EV touring problem, which is a generalization of the travelling salesman problem.

\subsection{A linear-time algorithm for finding optimal vehicle refuelling policies} 
\cite{honglinLineartimeAlgorithmFinding2007}
This explores a fixed-route vehicle refuelling problem as a special case of the inventory-capacitated lot-sizing problem. The authors present a linear-time greedy algorithm for finding optimal refuelling policies. The paper defines the "LOW function", which is used to compute the optimal refuelling policy. The authors provide two linear-time algorithms for the computation of the functions together with proofs of algorithmic correctness and computational efficiency. The paper concludes that an optimal refuelling policy always exists, and the amount of fuel left when arriving at the destination station is of no concern. The novelty of this paper lies in developing a linear-time greedy algorithm for finding optimal refuelling policies, which can be applied to real-world transportation problems.

\subsection{A fast algorithm for the gas station problem}
\cite{papadopoulosFastAlgorithmGas2018}
This paper presents an algorithm to solve the gas station problem, which involves finding the cheapest path between two vertices of an n-vertex graph while considering the fuel cost at each vertex and the car's fuel capacity. The algorithm improves upon the paper by Khuller, Malekian, and Mestre and has a time complexity of $O(n^2 + n^2 log n)$. 

\subsection{Reinforcement learning for the travelling salesman problem with refuelling}
\cite{ottoniReinforcementLearningTraveling2022}
They solve the TSPWR (Travelling Salesman Problem With Refuelling) using RL. Specifically 2 methods: SARSA and Q-learning. They analyse how the RL parameters and refuelling problem characteristics influence learning routes. Then they propose the use of the DQN algorithm to solve this problem. The proposed DQN-based approach is evaluated on benchmark instances of the TSPr. The results are compared with traditional exact and heuristic algorithms to showcase the effectiveness and efficiency of the RL-based method. The experimental results demonstrate that the DQN-based approach can find near-optimal solutions for the TSPr while effectively considering refuelling constraints. It outperforms traditional heuristics, especially for larger instances of the problem.

\subsection{Joint Optimization and Online Algorithms of Fuel-Aware Multiobjective Routing for Autonomous Vehicles}


\subsection{Online Routing for Autonomous Vehicle Cruise Systems with Fuel Constraints}
\cite{liOnlineRoutingAutonomous2022}
This paper addresses the "uninterrupted cruising" requirements for autonomous vehicles and the influence of limited fuel capacity on routing policies. They propose a heuristic solution by applying the fuel constraints iteratively on the shortest path that they say can be obtained in polynomial time. They also design a sliding-window-based algorithm for online routing, which allows a trade-off  between routing efficiency and computational complexity by adjusting the window size. Simulation results show that their proposed scheme reduces computation complexity by at least 13 times and improves performance by about 7\% in fuel consumption compared to alternative algorithms.

\subsection{Optimal Recharging Policies for Electric Vehicles}
\cite{swedaOptimalRechargingPolicies2017}
This paper addresses finding an optimal recharging policy for electric vehicles (EVs) along a given path. The authors address the problem of recharging decisions for EVs, which require special considerations due to battery dynamics. They present efficient algorithms for finding an optimal policy in general instances with deterministic travel costs and homogeneous charging stations, as well as for two specialized cases. The authors also develop two heuristic procedures that they characterize analytically and explore empirically. The paper further analyzes and tests the solution methods on model variations, including stochastic travel costs and nonhomogeneous charging stations. The contribution of this paper is the first effort in the literature to optimize recharging behavior for EVs.

\subsection{Optimal Routing of Energy-Aware Vehicles in Transportation Networks With Inhomogeneous Charging Nodes}
\cite{pourazarmOptimalRoutingEnergyAware2018}
This paper studies the problem of routing for energy-aware battery-powered vehicles (BPVs) in networks with charging nodes. The objective is to minimize the total elapsed time, including travel and recharging time at charging stations, so that the vehicle reaches its destination without running out of energy. The paper investigates the routing problem for BPVs through a network of "inhomogeneous" charging nodes. The paper studies two versions of the problem: the single-vehicle (user-centric) routing problem and the multiple-vehicle (system-centric) routing problem. For the former, the paper formulates a mixed-integer nonlinear programming (NLP) problem for simultaneously obtaining an optimal path and charging policy. The paper then reduces its computational complexity by decomposing it into two linear programming problems. For the latter, the paper uses a similar approach by grouping vehicles into "sub-flows" and formulating the problem at a sub-flow level with the inclusion of traffic congestion effects. The paper also proposes an alternative NLP formulation obtaining near-optimal solutions with orders of magnitude reduction in the computation time. The paper applies the optimal routing approach to a subnetwork of the eastern Massachusetts transportation network using actual traffic data provided by the Boston Region Metropolitan Planning Organization. Using these data, the paper estimates cost (congestion) functions and investigates the optimal solutions obtained under different charging stations and energy-aware vehicle loads.

\subsection{Finding Optimal Refueling Policies in Transportation Networks}
\cite{linFindingOptimalRefueling}
The authors analyze the optimal $[L,L]$ refuelling policies, that is the policies required to begin with a fuel level at the lower limit $L$, and end with a fuel level at least at the lower limit $L$. They prove that finding optimal $[L, L]$ vehicle refuelling policies in a transportation network is equivalent to finding the shortest paths in an optimal transition graph derived from the network. Devise algorithm to determine the optimal policy for all pairs of vertices in a network of n vertices in $O(n^3)$ and $O(n^3log(k))$ time where $k$ is the number of stops.





==> MIP.tex <==
\section{Mixed Integer Programming Formulation}
\label{ppwr:sec:mip}
We introduce a simple Mixed Integer Programming formulation to solve the \abbrPFRF. We borrow the formulation from~\cite{liaoElectricVehicleTouring2016}. However, we made some modifications since the formulation given in~\cite{liaoElectricVehicleTouring2016} is for a complete graph, which is not a requirement for us. Given an undirected graph $G =(V, E)$, where the vertices, $u \in V$ represent gas stations and edges $(u, v) \in E$ denote actions transiting the robot from vertex $u$ to $v$, a source vertex $v_o$ and a goal vertex $v_g$ (where $1\leq v_o, v_g \leq n$). Each edge is associated with a non-negative real value $d_{uv} \in \mathbb{R}^+ $, representing the fuel required to travel from vertex $u$ to $v$. Each vertex is associated with a cost $c(u)$, representing the cost of refuelling at vertex $u$, a variable $r_u$ referring to the amount of gas left in the tank, and $g_u$ referring to the amount of gas refuelled at the vertex. A binary variable $x_{uv}$ indicates if a path passes through the edge from $v_{u}$ to $v_{v}$. The robot has a maximum tank capacity of $q_{max}$. 
The objective given in ~\ref{mip_obj} is to minimize the cost of the total amount of gas purchased subject to constraints~\ref{mip_2},..,~\ref{mip_9}. Constraint~\ref{mip_2} forms a path from vertex $v_o$ to $v_g$, and constraint~\ref{mip_3} guarantees gas conservation through every edge. The tank capacity is ensured through constraint~\ref{mip_4}. Constraint~\ref{mip_5} introduces a binary variable~\ref{mip_5}, which denotes if refuelling happened at vertex $u$, and constraint~\ref{mip_6} ensures that the robot does not make more than $k_{max}$ stops. The robot begins with $0$ gas in its tank, shown in constraint~\ref{mip_8}.

\begin{align*}
\label{mip_eqns}
&  Min\left(\sum c(u)*g_u\right) \tag{1}\label{mip_obj}\\
& \sum x_{uv} - \sum x_{vu} = 
\begin{cases} 
1, & u=v_o;\\
-1, & u=v_g; \\
0, & \text{otherwise}
\end{cases} \;\; u = 1,2, \cdots, n \tag{2}\label{mip_2}\\
& (r_{u}+g_{u} -d_{uv} - r_v)*x_{uv} = 0, \;\; (v_{u}, v_{v})\; \in E \tag{3}\label{mip_3}\\
& r_{u}+g_{u}\leq q_{max} \tag{4}\label{mip_4}\\
& y_{rf} = 
\begin{cases} 
1, & g_{u} >0\\ 
0, & g_{u}= 0
\end{cases} \tag{5}\label{mip_5}\\
& \sum y_{rf} \leq k_{\max} \tag{6}\label{mip_6}\\
& x_{uv} \in \{0, 1\} \tag{7}\label{mip_7}\\
& r_{o}= q_{o} = 0 \tag{8}\label{mip_8}\\
& r_{u}, g_{u} \geq 0 \tag{9}\label{mip_9}\\
\end{align*}

==> Method/Unbounded_stops.tex <==
\subsection{Unbounded Number of stops Case :}
\label{ppwr:sec:Method:unbounded_stops}
In this subsection, we show how \abbrRAstar can be applied on a variant of the \abbrPFRF problem with stops mentioned in~\cite{khullerFillNotFill2011}, where there is no restriction on the number of stops the robot can make along an optimal path from $v_o$ to $v_g$. In their work, Khuller et al.~\cite{khullerFillNotFill2011} provide a modified dynamic programming (DP) formulation tailored for this variant, eliminating the need to account for the number of stops and thereby reducing the total state space. To adapt \abbrRAstar to this variant, slight adjustments are made to the algorithm. Simple modifications to Alg.~\ref{ppwr:alg:refuelA} include removing the check for $k_{max}$ in Line~\ref{alg1:line:kmaxCheck} and in  Alg.~\ref{ppwr:alg:checkPrune} the dominance check in Line~\ref{alg3:line:DomCheck} is altered and scalarized  to be $g(l') + (q(l) - q(l'))*c(v) \leq g(l)$. By doing so, \abbrRAstar only determines whether the robot has reached its goal. The dominance check, as mentioned in Def.~\ref{ppwr:def:dominance} reduces to only look for whether $q(l) \geq q(l')$ and $g(l) \leq g(l')$ and the check for stops are removed.

==> greedy.tex <==
\section{Greedy Formulation}
\label{ppwr:sec:greedy}
We also developed a greedy formulation~\cite{} to solve the \abbrPFRF, in a fast manner. However, we do not consider the number of stops made here and try to find a min-cost path $\pi(v_o, v_g)$ as quickly as possible. 
Here, the aim is to minimize the cost at every vertex. Let the robot be at vertex $u$ with neighbouring vertices $v$ and $k$, with refuelling costs $c(u), c(v) $ and $c(k)$, fuel needed to traverse from $u$ to $v$ and $k$ as $d_{uv}$ and $d_{uk}$, and fuel left at vertex $u$ as $q_u$. The greedy choice at any vertex $u$ that the robot has to make to go to the next gas station is given in equation~\ref{greedy_eqn}.

\begin{align}
\text{Next gas station} = 
\begin{cases}\label{greedy_eqn} 
    d_{uv} \leq q_{u}, & \text{go to } v;\\
    d_{uv} \leq d_{uk}, & \text{go to } v; \\
    \text{otherwise}, & \text{go to } k;
\end{cases}    \tag{10}
\end{align}

==> result/Frontier_vs_SP_plot.tex <==
\begin{figure}[h]
    % \vspace{-1em}
  \centering
  \includegraphics[scale=0.5]{Pics/FS_SPS_comp.png}
    \vspace{-1em}
  \caption{\small
  $\log - \log$ plot for size comparison between the size of the mean of the total frontier set size of \abbrRAstar calculated over 20 tests and the mean of the total state space size of the DP baseline.}
  \label{fig:FS_SP_plot}
    \vspace{-1.5em}
\end{figure}


==> result/Greedy.tex <==
\subsubsection{Greedy Formulation}
\label{ppwr:sec:results:greedy}
We also developed a greedy formulation~\cite{} to solve the \abbrPFRF, in a fast manner. However, we do not consider the number of stops made here and try to find a min-cost path $\pi(v_o, v_g)$ as quickly as possible. 
Here, the aim is to minimize the cost at every vertex. Let the robot be at vertex $u$ with neighbouring vertices $v$ and $k$, with refuelling costs $c(u), c(v) $ and $c(k)$, fuel needed to traverse from $u$ to $v$ and $k$ as $d_{uv}$ and $d_{uk}$, and fuel left at vertex $u$ as $q_u$. The greedy choice at any vertex $u$ that the robot has to make to go to the next gas station is given in equation~\ref{greedy_eqn}.

\begin{align}
\text{Next gas station} = 
\begin{cases}\label{greedy_eqn} 
    d_{uv} \leq q_{u}, & \text{go to } v;\\
    d_{uv} \leq d_{uk}, & \text{go to } v; \\
    \text{otherwise}, & \text{go to } k;
\end{cases}    \tag{10}
\end{align}

==> result/MICP.tex <==
\subsection{Mixed Integer Programming Formulation} \label{ppwr:sec:results:mip}
We introduce a simple Mixed Integer Programming formulation as an alternative baseline to solve the \abbrPFRF.
A binary variable $x(u, v)$ indicates if a path passes through the edge from $u$ to $v$, 
and binary variable $y(u)$ indicates whether the robot refuels at the vertex $u$.
Decision variables $a(u),q(u)$ are introduced in section~\ref{ppwr:sec:problem_state}.
The objective function in~Eq.\ref{res:mip_obj} is the total fuel cost along the path 
(borrowed from section~\ref{ppwr:sec:problem_state}), and is to be minimized.
Eq.~\eqref{res:vars} and Eq.~\eqref{res:mip_y} define the domain of decision variables.
Eq.~\eqref{res:stop_constr} defines the limit on the refuel stops, 
and Eq.~\eqref{res:flow_constr} defines the path from $v_o$ to $v_g$.
Eq.~\eqref{res:gas_conservation} indicates that if an edge $(u, v)$ is on the path, i.e.,
$x(u, v)=1$, then the remaining fuel at $v$ must be equal to the remaining fuel at $u$ plus 
the amount of refuelling at $u$, minus the consumption on the edge. 
Eq.~\eqref{res:smart_refuel} expresses the optimal refuelling strategy in Lemma~\ref{ppwr:lemma1}.

\begin{equation}\label{res:mip_obj}
	\min_{a(u),q(u),x(u,v)}\left(\sum c(u)a(u)\right)
\end{equation}

\begin{equation}\label{res:vars}
\begin{aligned}
	x(u,v) &\in \{0, 1\} \\
	q(u), a(u) &\geq 0 \\
	q(o) & = 0 \\
	q(u)+a(u) &\leq q_{max}\\
\end{aligned}
\end{equation}

\begin{equation} \label{res:mip_y}
		y(u) = 
	\begin{cases} 
	 1, & a(u) > 0 \\ 
	 0, & a(u) = 0
	 \end{cases}\\
\end{equation}

\begin{equation}\label{res:stop_constr}
	\sum_{u\in V} y(u) \leq k_{\max}
\end{equation}

\begin{equation}\label{res:flow_constr}
	\sum_{v\in V} x(u,v) - \sum_{v\in V} x(v,u) = 
 \begin{cases} 
 1, & u=v_o;\\
 -1, & u=v_g; \\
 0, & u\in V/\{v_o,v_g\}
 \end{cases}
\end{equation}

\begin{equation}\label{res:gas_conservation}
(q(u)+a(u) -d(u,v) - q(v))x(u,v) = 0, \;\; (u, v)\; \in E 
\end{equation}

\begin{equation}\label{res:smart_refuel}
	\begin{aligned}
		\forall x(u, v) = 1\;, (u, v)\in E,\;\\
	\begin{cases}
		a(u) = q_{max}, & c(u)<c(v)\\
		a(u) + q(u) \geq d(u, v), & c(u)\geq c(v)\\
	\end{cases}
	\end{aligned}
\end{equation}


==> result/RT_plot.tex <==
% \begin{figure*}[t]
%   \centering
%   \includegraphics[width=\textwidth]{source/Pics/rt_fs_sp_size_plots.png} 
%   \caption{Both figures are log-log plots for comparison between \abbrRAstar and DP baseline.
%   (a) showcases the mean run times and the variance plots. (b) is a plot of the size of the median $\FrontierSet$ size and median state-space size.}
%   \label{fig:result_plots}
% \end{figure*}

\begin{figure}[ht]
  \centering
  \includegraphics[scale=0.5]{Pics/RT_comp.png} 
    \vspace{-1em}
  \caption{\small
  $\log - \log$ plot for runtime (s) comparison between \abbrRAstar and DP baseline}
  \vspace{-1.5em}
  \label{fig:RT_plot}
\end{figure}



==> result/heu_per.tex <==
\begin{figure}[htbp]
    % \vspace{-1em}
  \centering
  \includegraphics[scale=0.5]{Pics/heu_per.png} 
    \vspace{-1em}
  \caption{\small
  $\log$-plot of the run-time comparison for \abbrRAstar when heuristic influence is varied from $0-100 \%$, and a variant of the DP algorithm with a termination condition for when the goal vertex is reached.}
  \label{fig:heu_per}
    \vspace{-1.5em}
\end{figure}


==> result/result.tex <==
\section{Results}
\label{ppwr:sec:results}
\subsection{Testing and implementation}
\label{ppwr:sec:results:testing_det}
We compare our \abbrRAstar against the DP method\cite{khullerFillNotFill2011}. Both are implemented in C++17 and tested on a Ubuntu 20.04 laptop with AMD Ryzen 7 4800h 4.3GHz CPU and 16GB RAM.
\begin{figure}[t]
  \centering
  \includegraphics[width=\columnwidth]
  {Pics/phil_src_dest_plot.png} 
    \vspace{-1em}
  \caption{
  \small
  Visualization of the map for Philadelphia, PA, USA, used in testing. (a) showcases the city road network of Philadelphia, where the red dots represent the gas stations. 
  We create a ``gas station graph'' $G=(V, E)$ for our tests, where $V$ is the set of gas stations, and each edge is a minimum cost path between the corresponding gas stations.
  We create this graph $G$ using a pre-processing step, and both algorithms (\abbrRAstar and DP) runs on this $G$ as opposed to the original city road network.
  (b) shows the solution path returned by our algorithm for one such test case. The agent stops at 5 gas stations before reaching the destination.}
  \label{fig:wide_image}
  \vspace{-1.5em}
\end{figure}

\subsubsection{Data preparation and testing}
We use graphs from \textit{OpenStreetMap} dataset over the USA and Europe, collected using the ``\textit{osmnx}" library in Python. The cities used with the number of gas stations: Philadelphia, PA, USA (61); Austin, TX, USA (87); Phoenix, AZ, USA (178); London, UK (258); and Moscow, Russia (423). 
% Querying the map data is done using the Python library, after which the vertex (gas station) IDs, distances between every pair of vertices (calculated using Dijkstra) and the costs (taken from a normal distribution generated from the means and standard deviations of gas prices) is extracted into ``.csv'' files, which are shared in our GitHub repository for reference.
We use 20 random start-goal pairs in each city for testing.
% The comparison is given in Fig.~\ref{fig:RT_plot},~\ref{fig:FS_SP_plot}.

%% Add the MIP and the greedy baselines as sub-sub sections 2 and 3 here.

\input{result/RT_plot}
\input{result/Frontier_vs_SP_plot}
\input{result/heu_per}

\subsection{Discussion}
\label{ppwr:sec:results:discussion}
From the numerical results shown in Fig.~\ref{fig:RT_plot}, we can see that our algorithm \abbrRAstar takes significantly less time than the DP baseline~\cite{khullerFillNotFill2011} to execute and find an optimal solution. The properties of our algorithm which allow for such fast computation are mainly due to the heuristic function, not constructing and exploring the entire search space and the dominance rules, which are explained as follows.


\subsubsection{Runtime comparison}
\abbrRAstar expedites the computational by avoiding constructing the entire state space. \abbrRAstar selectively explores the necessary labels for expansion and prunes the labels which get dominated. \abbrRAstar becomes increasingly advantageous when searching larger graphs. As seen in Fig.~\ref{fig:RT_plot} on the graph with 400+ stations, \abbrRAstar achieved a mean run-time of roughly $1s$, whereas the DP took more than $1000s$.


\subsubsection{Search space exploration}
The heuristic-guided nature of our algorithm directs the search process towards more promising areas of the state space. The dominance rule introduced in Def.~\ref{ppwr:def:dominance} prunes labels during the search process, expanding fewer labels and reducing the space's size. Hence minimizing unnecessary exploration. From Fig.~\ref{fig:FS_SP_plot}, we can see that the total size of the frontier set, i.e., the sum of the frontier set at all vertices explored, is approximately $10$ times smaller than the DP's state space size. This addition helps reduce the computational overhead and keeps the set of paths to be explored (stored in $\FrontierSet$) to a minimum, unlike DP, which constructs the entire state space.  


\subsubsection{Influence of heuristic}
% \abbrRAstar considers both heuristics and dominance pruning to expedite the computation.
To understand the effect of using the heuristic, we further introduce two variants of the methods.
The first variant is based on the DP method, where the computation terminates immediately after an optimal start-goal path is found, as opposed to computing $A(v,q,k)$ for all states as mentioned in~\cite{khullerFillNotFill2011}.
The second variant is based on \abbrRAstar, where the ``guiding power'' of the heuristic is reduced by multiplying $h$-values with a weight factor from $[0,1]$.
By doing so, we seek to verify the benefit of using a heuristic to guide the search when solving \abbrPFRF.
We used Phoenix, AZ, USA, with 178 gas stations in this test, and conducted tests on 20 randomly generated start-goal pairs.
% In this test, we fixed the map to Phoenix, AZ, USA, which has 178 gas stations. The tests were conducted on 20 randomly generated start-goal pairs.

Fig.~\ref{fig:heu_per} shows the runtime of both DP with entire state-space creation as $78s$, and DP with early termination as $60s$.
Allowing early termination of DP after finding the optimal start-goal path helps reduce the algorithm's runtime.
However, the DP computation is still expensive compared to the \abbrRAstar method, since \abbrRAstar avoids the explicit state space construction and can use dominance pruning during the search.
We also observe that, for \abbrRAstar, the heuristic can expedite the computation from nearly $1s$ to roughly $0.25s$, which shows the benefit of using a heuristic.

% . The figure also provides a case for a variant of the DP baseline, wherein we eschew the computation by forgoing the construction of the entire state space.
% Instead, we ask the search to terminate once the goal station is reached. Fig. ~\ref{fig:heu_per} shows a noticeable reduction in the run-times of both variants, when we construct the entire state-space and when we do not.

% Mention the influence of heuristic information on performance. Add a graph -> percentage of the heuristic (0-20-40-60-80-100%). 200 stations case. Report the run-time. 

